Point Cloud Completion by Learning Shape Priors

In view of the difficulty in reconstructing object details in point cloud completion, we propose a shape prior learning method for object completion. The shape priors include geometric information in both complete and the partial point clouds. We design a feature alignment strategy to learn the shape prior from complete points, and a coarse to fine strategy to incorporate partial prior in the fine stage. To learn the complete objects prior, we first train a point cloud auto-encoder to extract the latent embeddings from complete points. Then we learn a mapping to transfer the point features from partial points to that of the complete points by optimizing feature alignment losses. The feature alignment losses consist of a L2 distance and an adversarial loss obtained by Maximum Mean Discrepancy Generative Adversarial Network (MMD-GAN). The L2 distance optimizes the partial features towards the complete ones in the feature space, and MMD-GAN decreases the statistical distance of two point features in a Reproducing Kernel Hilbert Space. We achieve state-of-the-art performances on the point cloud completion task. Our code is available at https://github.com/xiaogangw/point-cloud-completion-shape-prior.

==> table_paper/fpd_values.tex <==
\begin{table*}[!htbp]
\small
\centering
\caption{CD ($10^{-4}$) and FPD comparison among different methods. The lower the better.} 
\vspace{-0.2cm}
\resizebox{0.90\textwidth}{!}{
\begin{tabular}{l|c| c| c| c| c|c| c| c} %| c | c
\hline
Method &  PCN~\cite{yuan2018pcn} & TopNet~\cite{topnet2019} &  PCN~\cite{yuan2018pcn} + L2 &PCN~\cite{yuan2018pcn} + LS &PCN~\cite{yuan2018pcn} + MMD & Ours-L2 & Ours-LS & Ours-MMD \\ 
\hline
CD  &9.02 &9.88 & 8.38 &8.54 &8.46 &7.42 &7.59 &\textbf{7.39}\\   %&8.93 
FPD &7.91 &9.43 &7.06 &5.87 &7.26 &\textbf{5.74} &6.46 &5.97\\   %&8.93 
\hline
\end{tabular}
}
\vspace{-0.4cm}
\label{fpd_values}
\end{table*}
